Anatomy of Graph Matching based on an XQuery and RDF Implementation

Graphs are becoming one of the most popular data modeling paradigms since they are able to model complex relationships that cannot be easily captured using traditional data models. One of the major tasks of graph management is graph matching, which aims to find all of the subgraphs in a data graph that match a query graph. In the literature, proposals in this context are classified into two different categories: graph-at-a-time, which process the whole query graph at the same time, and vertex-at-a-time, which process a single vertex of the query graph at the same time. In this paper, we propose a new vertex-at-a-time proposal that is based on graphlets, each of which comprises a vertex of a graph, all of the immediate neighbors of that vertex, and all of the edges that relate those neighbors. Furthermore, we also use the concept of minimum hub covers, each of which comprises a subset of vertices in the query graph that account for all of the edges in that graph. We present the algorithms of our proposal and describe an implementation based on XQuery and RDF. Our evaluation results show that our proposal is appealing to perform graph matching.

==> macros/Dirty-Tricks.tex <==
% Dirty-Tricks.tex

\RequirePackage{macros/mathident}

% Legends to tables

\newenvironment{legend}{%
    \trivlist\item\footnotesize
}{%
    \endtrivlist
}

% This provides a few patches that make the LLNCS class more `human-friendly' :)

\AtBeginDocument{
    \def\figurename{Figure}

    \pagestyle{plain}

    \let\saveparagraph=\paragraph
    \def\paragraph#1{\saveparagraph{\bfseries #1}}

    \let\savecaption=\caption
    \def\caption#1{\smallbreak\savecaption{#1}}

    \let\savefigure=\figure
    \def\figure{\savefigure \centering\small}

    \let\savetable=\table
    \def\table{\savetable \centering\small}
}

% This allows LaTeX to place floats a lot better.

\makeatletter
    \def\fps@figure{tbp}
    \def\fps@table{tbp}
    \renewcommand\ps@empty{\ps@plain}
    \setcounter{topnumber}{2}
    \setcounter{bottomnumber}{1}
    \setcounter{totalnumber}{3}
    \setcounter{dbltopnumber}{2}
    \renewcommand\topfraction{.85}
    \renewcommand\bottomfraction{.85}
    \renewcommand\dbltopfraction{.85}
    \renewcommand\textfraction{.1}
    \renewcommand\floatpagefraction{.85}
    \renewcommand\dblfloatpagefraction{.85}
\makeatother



==> src/analysis.tex <==
\section{Analysis}
\label{sec:analysis}

\begin{definition}
\label{def:state-space}
Let $G$ and $Q$ be two graphs, and $O$ an ordering of the vertices of $Q$. A state space is the set of all partial solutions that algorithm $findSolutions$ explores to find the solutions of $Q$ over $G$ using $O$. We denote this state space as $\Psi(G, Q, O)$.
\end{definition}

\begin{definition}
\label{def:inner-ordering}
Let $Q$ be a graph, $O$ an ordering of the vertices of $Q$, and $O'$ an ordering of a subset of the vertices of $Q$. $O'$ is an inner ordering of $O$ if $O' \subseteq O$, and the vertices in $O'$ appear in the same order as in $O$.
\end{definition}

\begin{theorem}
\label{theo:partial-solutions}
Let $G$ and $Q$ be two graphs, $O$ an ordering of the vertices of $Q$, and $O'$ an inner ordering of the vertices of $M \subseteq MHC(Q)$ such that $M \subseteq Q$. The partial solutions computed by algorithm $findSolutions$ using $O$ are included in the partial solutions computed by algorithm $findSolutions$ using $O'$.
\end{theorem}

\begin{proof}
Let $\Psi(G, Q, O)$ and $\Psi(G, Q, O')$ be the state spaces of algorithm $findSolutions$ using $O$ and $O'$, respectively. The proof follows from reductio ad absurdum: assume that there exists a partial solution $s \in \Psi(G, Q, O')$ such that $s \notin \Psi(G, Q, O)$. If this occurs, it is because there exists a pair $(k = v)$, in which $k \in vertices(Q)$ and $v \in vertices(G)$, such that it does not belong to any partial solution in $\Psi(G, Q, O)$.

To compute $(k = v)$, algorithm $findSolutions$ unifies $G$ and $q$, which is the graphlet that results from substituting it using the previous partial solution $current$ (see lines~\ref{line:find-solutions:get-graphlet}--~\ref{line:find-solutions:unify} in Figure~\ref{fig:find-solutions}). Since $current$ belongs to both $\Psi(G, Q, O)$ and $\Psi(G, Q, O')$, $q$ is also computed when calling algorithm $findSolutions$ using $O$. Therefore, the same set of partial solutions are computed when unifying $G$ and $q$, in which $(k = v)$ belongs to one or more partial solutions in $\Psi(G, Q, O)$, and $s \in \Psi(G, Q, O)$, which is a contradiction. As a conclusion, the partial solutions computed by algorithm $findSolutions$ using $O$ are included in the partial solutions computed by algorithm $findSolutions$ using $O'$.
\end{proof} 
